Diffeomorphic Image Registration with Neural Velocity Field

Diffeomorphic image registration, offering smooth transformation and topology preservation, is required in many medical image analysis tasks.Traditional methods impose certain modeling constraints on the space of admissible transformations and use optimization to find the optimal transformation between two images. Specifying the right space of admissible transformations is challenging: the registration quality can be poor if the space is too restrictive, while the optimization can be hard to solve if the space is too general. Recent learning-based methods, utilizing deep neural networks to learn the transformation directly, achieve fast inference, but face challenges in accuracy due to the difficulties in capturing the small local deformations and generalization ability. Here we propose a new optimization-based method named DNVF (Diffeomorphic Image Registration with Neural Velocity Field) which utilizes deep neural network to model the space of admissible transformations. A multilayer perceptron (MLP) with sinusoidal activation function is used to represent the continuous velocity field and assigns a velocity vector to every point in space, providing the flexibility of modeling complex deformations as well as the convenience of optimization. Moreover, we propose a cascaded image registration framework (Cas-DNVF) by combining the benefits of both optimization and learning based methods, where a fully convolutional neural network (FCN) is trained to predict the initial deformation, followed by DNVF for further refinement. Experiments on two large-scale 3D MR brain scan datasets demonstrate that our proposed methods significantly outperform the state-of-the-art registration methods.

==> abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
   Diffeomorphic image registration, requiring the transformation to be smooth with smooth inverse, is an essential task in many medical image analysis problems.
   %
   Traditional optimization-based methods impose certain modeling constraints on the space of permissible transformations and use optimization to identify the optimal transformation between two images. Specifying the right space of permissible transformations is challenging: if the space is too restrictive, the registration quality can be poor; if the space is too general, the optimization can be hard to solve. 
   %
  %   , and a trade-off exists between speed and accuracy. 
Recent learning-based methods, utilizing deep neural networks to learn the transformation directly, achieve fast inference speed, but face challenges in deformation accuracy due to the difficulties in capturing the small local deformations and generalizability issues associated with new data. 
%   
Here we propose a new optimization-based method named DNVF (\underline{D}iffeomorphic image registration with \underline{N}eural \underline{V}elocity \underline{F}ield).
%
DNVF uses deep neural nets to model the space of permissible transformations between two images, providing the flexibility of modeling complex deformations as well as the convenience of optimization. To produce diffeomorphic registration, DNVF uses a multilayer perceptron (MLP) to model a continuous velocity field, taking a 3D coordinate as input and outputting the corresponding velocity vector at the location. 
%
% utilizes an implicit neural representation of a continuous velocity field to describe the diffeomorphic deformation across two images. Specifically, for each spatial point, DNVF takes the 3D coordinate as input and assigns the corresponding velocity vector through a multilayer perceptron (MLP), which has higher flexibility and modeling power than traditional methods. 
Having the periodic sinusoidal function as the activation layer enables the network to model complex deformatiosn by fitting high frequency content and also enables quick convergence. 
%
Moreover, we propose a cascaded image registration framework (Cas-DNVF), where we train a fully convolutional neural network (FCN) to predict an initial deformation, followed by DNVF to further refine the transformation. Cas-DNVF combines the benefits of both optimization and learning based methods, with fast inference while maintaining good registration accuracy and model generalization. 
%simplifies the search space of optimal deformations so that DNVF can focus on modeling hard local residual deformations more efficiently. 
%
Extensive experiments conducted on two large-scale 3D MR brain scan datasets demonstrate that our proposed methods outperform the state-of-the-art registration methods by a large margin. 
\end{abstract}



